Inferring Individual Direct Causal Effects Under Heterogeneous Peer Influence

Causal inference in networks should account for interference, which occurs when a unit's outcome is influenced by treatments or outcomes of peers. Heterogeneous peer influence (HPI) occurs when a unit's outcome is influenced differently by different peers based on their attributes and relationships, or when each unit has a different susceptibility to peer influence. Existing solutions to estimating direct causal effects under interference consider either homogeneous influence from peers or specific heterogeneous influence mechanisms (e.g., based on local neighborhood structure). This paper presents a methodology for estimating individual direct causal effects in the presence of HPI where the mechanism of influence is not known a priori. We propose a structural causal model for networks that can capture different possible assumptions about network structure, interference conditions, and causal dependence and enables reasoning about identifiability in the presence of HPI. We find potential heterogeneous contexts using the causal model and propose a novel graph neural network-based estimator to estimate individual direct causal effects. We show that state-of-the-art methods for individual direct effect estimation produce biased results in the presence of HPI, and that our proposed estimator is robust.

==> graphs/01-example-socialnetwork.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,235); %set diagram left start at 0, and has height of 235

%Shape: Rectangle [id:dp29447453031599724] 
\draw   (332,64) -- (459,64) -- (459,192.19) -- (332,192.19) -- cycle ;
%Shape: Diamond [id:dp7825919997893931] 
\draw   (268,94) -- (314,129) -- (268,164) -- (222,129) -- cycle ;
%Curve Lines [id:da9619201968698301] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (268,164) .. controls (269,182) and (284,177) .. (334,178) ;
%Curve Lines [id:da0006560377031847864] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (268,94) .. controls (271,75) and (283,82) .. (332,82) ;
%Shape: Ellipse [id:dp5674777077210205] 
\draw   (351,90.5) .. controls (351,83.04) and (371.37,77) .. (396.5,77) .. controls (421.63,77) and (442,83.04) .. (442,90.5) .. controls (442,97.96) and (421.63,104) .. (396.5,104) .. controls (371.37,104) and (351,97.96) .. (351,90.5) -- cycle ;
%Shape: Ellipse [id:dp44396094118221097] 
\draw   (352,130.5) .. controls (352,123.04) and (372.37,117) .. (397.5,117) .. controls (422.63,117) and (443,123.04) .. (443,130.5) .. controls (443,137.96) and (422.63,144) .. (397.5,144) .. controls (372.37,144) and (352,137.96) .. (352,130.5) -- cycle ;
%Shape: Ellipse [id:dp5094888669208908] 
\draw   (346,167.5) .. controls (346,160.04) and (369.06,154) .. (397.5,154) .. controls (425.94,154) and (449,160.04) .. (449,167.5) .. controls (449,174.96) and (425.94,181) .. (397.5,181) .. controls (369.06,181) and (346,174.96) .. (346,167.5) -- cycle ;


% Text Node
\draw (361,42) node [anchor=north west][inner sep=0.75pt]   [align=left] {USER $\displaystyle ( U)$};
% Text Node
\draw (204.05,39.85) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.36] [align=left] {FOLLOWS($\displaystyle U_{1} ,U_{2})$};
% Text Node
\draw    (268, 128.5) circle [x radius= 29.7, y radius= 14.85]   ;
\draw (248,120) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{28.24pt}\setlength\topsep{0pt}
\begin{center}
Since
\end{center}

\end{minipage}};
% Text Node
\draw (363,83) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Disposition};
% Text Node
\draw (355,160) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {PrivacySetting};
% Text Node
\draw (363,124) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {TimeOnSite};


\end{tikzpicture}

==> graphs/Brainstorming.tex <==
% \textbf{Representation of Heterogenity in SCM}
% \begin{itemize}
% \item Non-parametric nature of SCM with V = f(pa(V)), shows potential interactions i.e. heterogeneity
% \item Actual heterogeneity detection depends on model parameters $\displaystyle \theta $
% \item Estimands for c-specific effects with SCM structure (Pearl)
% \item Latent heterogeneity due to unobserved interactions (Pearl)
% \item Four types of effect modifiers (Characterization with SCM)
% \begin{itemize}
% \item Direct effect modifiers (actual interaction)
% \item Indirect effect modifiers (Due to d-separation)
% \item Effect modifers due to proxies (Due to d-separation)
% \item Effect modifiers due to common causes (Due to d-separation)
% \end{itemize}
% \item Given treatment (T) and outcome (O), the potential sources of interactions are parents of outcome and mediators that are non-descandants of Treatment
% \end{itemize}


% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,192); %set diagram left start at 0, and has height of 192

% %Shape: Ellipse [id:dp94065429660476] 
% \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (490,154) .. controls (490,149.03) and (498.28,145) .. (508.5,145) .. controls (518.72,145) and (527,149.03) .. (527,154) .. controls (527,158.97) and (518.72,163) .. (508.5,163) .. controls (498.28,163) and (490,158.97) .. (490,154) -- cycle ;
% %Shape: Ellipse [id:dp689008112234961] 
% \draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (489,177) .. controls (489,172.03) and (497.28,168) .. (507.5,168) .. controls (517.72,168) and (526,172.03) .. (526,177) .. controls (526,181.97) and (517.72,186) .. (507.5,186) .. controls (497.28,186) and (489,181.97) .. (489,177) -- cycle ;

% % Text Node
% \draw    (270, 33.5) circle [x radius= 50.91, y radius= 14.85]   ;
% \draw (235,25) node [anchor=north west][inner sep=0.75pt]   [align=left] {Treatment};
% % Text Node
% \draw    (269.5, 90.5) circle [x radius= 44.55, y radius= 14.85]   ;
% \draw (239,82) node [anchor=north west][inner sep=0.75pt]   [align=left] {Mediator};
% % Text Node
% \draw    (271.5, 145.5) circle [x radius= 45.96, y radius= 14.85]   ;
% \draw (240,137) node [anchor=north west][inner sep=0.75pt]   [align=left] {Outcome};
% % Text Node
% \draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (435, 92.5) circle [x radius= 111.72, y radius= 14.85]   ;
% \draw (357,84) node [anchor=north west][inner sep=0.75pt]   [align=left] {Direct Int with Mediator};
% % Text Node
% \draw    (435, 24.5) circle [x radius= 56.57, y radius= 14.85]   ;
% \draw (396,16) node [anchor=north west][inner sep=0.75pt]   [align=left] {Indirect EM};
% % Text Node
% \draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ]  (128.5, 61.5) circle [x radius= 118.09, y radius= 14.85]   ;
% \draw (46,53) node [anchor=north west][inner sep=0.75pt]   [align=left] {Direct Int with Treatment};
% % Text Node
% \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ]  (436.5, 143.5) circle [x radius= 48.79, y radius= 14.85]   ;
% \draw (403,135) node [anchor=north west][inner sep=0.75pt]   [align=left] {Proxy EM};
% % Text Node
% \draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ]  (547.5, 58.5) circle [x radius= 98.29, y radius= 14.85]   ;
% \draw (479,50) node [anchor=north west][inner sep=0.75pt]   [align=left] {Common Cause EM};
% % Text Node
% \draw (534,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {Non-causal EM};
% % Text Node
% \draw (534,168) node [anchor=north west][inner sep=0.75pt]   [align=left] {Actual Interaction};
% % Text Node
% \draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ]  (114, 115.5) circle [x radius= 84.85, y radius= 14.85]   ;
% \draw (55,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {Latent Interaction};
% % Connection
% \draw    (269.87,48.35) -- (269.65,73.65) ;
% \draw [shift={(269.63,75.65)}, rotate = 270.5] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% % Connection
% \draw    (270.04,105.35) -- (270.89,128.65) ;
% \draw [shift={(270.96,130.65)}, rotate = 267.92] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% % Connection
% \draw    (392.6,106.24) -- (305.85,134.37) ;
% \draw [shift={(303.95,134.98)}, rotate = 342.04] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% % Connection
% \draw    (190.11,74.17) -- (229.62,82.3) ;
% \draw [shift={(231.58,82.7)}, rotate = 191.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% % Connection
% \draw    (435,39.35) -- (435,75.65) ;
% \draw [shift={(435,77.65)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% % Connection
% \draw    (435.44,107.35) -- (436,126.65) ;
% \draw [shift={(436.06,128.65)}, rotate = 268.32] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% % Connection
% \draw    (472.1,35.71) -- (501.63,44.64) ;
% \draw [shift={(503.54,45.21)}, rotate = 196.82] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% % Connection
% \draw    (171.41,126.43) -- (229.94,137.58) ;
% \draw [shift={(231.9,137.96)}, rotate = 190.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% \end{tikzpicture}

% \textbf{Characterization of heterogeneity with SCM.}

% Three categories of effect modifications:
% \begin{itemize}
% \item Due to direct or mediated interaction with treatment
% \item Due to dependency with interacting variables
% \item Latent heterogeneity
% \end{itemize}

% \textbf{Heterogeneity with latent variables}
% \begin{itemize}
% \item If "Direct Interaction" variable is unobserved, "Proxy EM" may act as interacting variable. Additionaly, when Indirect EM is unobserved, "Common Cause EM" also acts as interacting variable.
% \item Interaction of treatment with latent variable.
% \item Pearl's detection of latent heterogeneity.
% \end{itemize}

% \textbf{Actual detection of interaction requires estimation. }
% \begin{itemize}
% \item Data-driven methods
% \item Model-driven methods
% \end{itemize}


% \textbf{Taking this idea to relational models.}
% \begin{itemize}
% \item With model we can find potential sources of hetergeneity
% \end{itemize}
% \newchange{\section{Discovering Causes and Effect Modifiers}\label{sec:pr_setup}}
% \newchange{In this section, we characterize the causes and effect modifiers of an outcome using the concepts of a structural causal model (SCM)~\cite{pearl-book09} and hypothetical interventional distribution, and formally define our research problems.}

% \newchange{A SCM {\small $\mathcal{M}(\mathbf{V}, \mathbf{U}, \mathbf{f})$} models the underlying causal data-generating mechanism with a set of exogenous variables {\small $\mathbf{U}$}, endogenous variables {\small $\mathbf{V}$}, and functions {\small $\mathbf{f}$}.
% % The exogenous variables {\small $\mathbf{U}$} are external to the causal model and considered errors or disturbances. 
% A variable is a function of its known direct causes {\small $\mathbf{V}$} and unknown disturbances {\small $\mathbf{U}$}.
% The causal relationship among the variables in an SCM is represented using a directed acyclic graph (DAG) {\small $G(\mathbf{V}, \mathbf{E})$} where {\small $\mathbf{V}$} and {\small $\mathbf{E}$} are a set of vertices and edges, respectively, and each vertex has incoming edges from its direct causes. 
% {\small $V_i \rightarrow V_j$} denotes an edge from the parent {\small $V_i$} to the child {\small $V_j$}.
% Two vertices are adjacent if there is an edge between them.
% A directed path is a sequence of nodes obtained following the direction of the edges. A graph is directed acyclic if there are no directed paths with repeated nodes. The nodes preceding the tail node of the directed path are the ancestors of the tail node. The nodes following the head node of the directed path are descendants of the head node.
% The symbols {\small $pa(V_i, G)$}, {\small $anc(V_i, G)$}, and {\small $des(V_i, G)$} indicate the sets of parents, ancestors, and descendants of {\small $V_i$} for graph {\small $G$}, respectively.
% }

% \newchange{Given an oracle SCM $G$, the causes of an outcome $Y$ are its ancestors, i.e., $anc(Y, G)$.
% %Let $X^j$ and $Y$ be the random variables for the $j^{th}$ event and the outcome respectively. 
% An event $X^j$ is a cause of outcome $Y$ if the conditional average treatment effect (CATE) for any context $\mathbf{Z}\subset \mathbf{V}| \mathbf{Z} \not\subset des(Y,G)$ is non-zero:
% % \fixme{
% {\small
% \begin{equation}\label{eq:ate}
% \begin{split}
%     \exists{\mathbf{Z}}, X^j_{CATE}(\mathbf{Z}=\mathbf{z}) :=
%     E[Y|do(X^{j}=x), \mathbf{Z}=\mathbf{z}] - \\E[Y|do(X^{j}=x'), \mathbf{Z}=\mathbf{z}] \ne 0,
% \end{split}
% \end{equation}}
% % }
% where {\small $do(X^j=x)$} and {\small $do(X^j=x')$} denote interventions to the value of {\small $X^j$} with a policies {\small $x$} and {\small $x'$}, respectively and {\small $\mathbf{Z}=\mathbf{z}$} is the context of the intervention that is non-descendant of outcome.
% % The estimand on Eq. \ref{eq:ate} assumes the variables $\mathbf{Z}$ are observed.
% The causal effect in Eq. 3 is measured on an additive scale. Sometimes, for a binary outcome, the effect may be measured on a multiplicative scale like a risk ratio or an odds ratio. A treatment may have heterogeneous effects on the outcome in different contexts $\mathbf{Z}$. These contexts are referred to as effect modifiers.}

% \newchange{
% %Next, we discuss how the problem of discovering effect modifiers relates to a SCM, particularly the causal graphical model $G$.
% A variable {\small $Z$} is an effect modifier for treatment {\small $X^j$} and outcome {\small $Y$} if CATE is different any two levels of {\small $Z$}.
% {\small
% \begin{equation}\label{eq:hte}
%     X^j_{CATE}(Z=z) \ne X^j_{CATE}(Z=z'),
% \end{equation}
% }
% where {\small $z$} and {\small $z'$} are two different assignments of {\small $Z$}.
% The presence of heterogeneity or effect modification actually depends on the functions $\mathbf{f}$ of the SCM. A context Z is an effect modifier of a treatment $X$ on an outcome $Y$ if a direct interaction between $X$ and $Z$ defines $Y$, i.e.,
% {\small
% % \begin{equation}\label{eq:em}
%     $Y=f_Y(g(h(X)*Z)),$
% % \end{equation}
% }
% where $*$ denotes interaction and $\{g,h\} \in \mathbf{f}$ are optional intermediate functions. Similarly, the non-linearity of $\mathbf{f}$ can introduce heterogeneity because effects are measured on an additive scale. For instance, a SCM $Y = relu (-1+X+2Z)$, with binary treatment $X$ and context $Z$, has CATEs of $0$ for $Z=0$ and $1$ for $Z=1$ due to rectified linear unit activation. We refer the effect modification by non-linearity alone as an indirect interaction.
% %While $G$ informs us about potential heterogeneity, the presence of heterogeneity is determined by the SCM's functions $\mathbf{f}$.
% }
% \begin{figure}[t]
%     \centering
%     \includegraphics[height=0.35\linewidth]{images/EffectModifiers.pdf}
%     \caption{Characterization of effect modifiers (EM) with a structural causal model (SCM).}
%     \label{fig:em}
%     \vspace{-1em}
% \end{figure}

% \newchange{Although the presence of effect modification is determined by the estimation of CATE (Eq. \ref{eq:hte}), the graphical structure $G$ can still inform potential effect modification. \citet{vanderweele-epi07} have studied identification and categorization of effect modifiers in causal graphs. Figure \ref{fig:em} summarizes our categorization of effect modification: (1) due to direct or mediated interactions with treatment, (2) due to dependency with interacting variables, and (3) due to latent interactions. The potential interacting variables for a given treatment and outcome in a $G$ include the non-descendants of the treatment node and either (1) the parents of the outcome or (2) the parents of mediator nodes in the directed path from treatment to outcome~\cite{vanderweele-epi07}.
% In a mediated interaction, the treatment X may be transformed by intermediate functions. As shown in Figure \ref{fig:em}, indirect, proxy, common cause, and selection bias effect modifiers are non-descendants of treatment with dependence to interacting variables via ancestor, descendant, confounding, and selection relations, respectively. There can be effect modifications due to interaction and dependency with latent variables.
% }




==> graphs/CannabisRelationalModel.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,347); %set diagram left start at 0, and has height of 347

%Shape: Rectangle [id:dp6061233253065852] 
\draw   (148,45) -- (379,45) -- (379,277) -- (148,277) -- cycle ;
%Shape: Ellipse [id:dp679503702340104] 
\draw   (190,77) .. controls (190,65.95) and (223.8,57) .. (265.5,57) .. controls (307.2,57) and (341,65.95) .. (341,77) .. controls (341,88.05) and (307.2,97) .. (265.5,97) .. controls (223.8,97) and (190,88.05) .. (190,77) -- cycle ;

%Shape: Ellipse [id:dp5368901700546405] 
\draw   (178,150.5) .. controls (178,135.86) and (216.95,124) .. (265,124) .. controls (313.05,124) and (352,135.86) .. (352,150.5) .. controls (352,165.14) and (313.05,177) .. (265,177) .. controls (216.95,177) and (178,165.14) .. (178,150.5) -- cycle ;

%Shape: Ellipse [id:dp15750704570277696] 
\draw   (178,234.5) .. controls (178,219.86) and (216.95,208) .. (265,208) .. controls (313.05,208) and (352,219.86) .. (352,234.5) .. controls (352,249.14) and (313.05,261) .. (265,261) .. controls (216.95,261) and (178,249.14) .. (178,234.5) -- cycle ;

%Straight Lines [id:da2354631484175722] 
\draw    (265.5,97) -- (265.06,121) ;
\draw [shift={(265,124)}, rotate = 271.06] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da9011938368445787] 
\draw    (265,177) -- (265,205) ;
\draw [shift={(265,208)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Curve Lines [id:da49514783253186767] 
\draw    (341,77) .. controls (376.28,132.86) and (368.34,194.48) .. (325.66,214.81) ;
\draw [shift={(323,216)}, rotate = 337.11] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Flowchart: Decision [id:dp44985849197324734] 
\draw   (79,121) -- (142,157) -- (79,193) -- (16,157) -- cycle ;
%Shape: Ellipse [id:dp9208736783238205] 
\draw   (46,157) .. controls (46,148.44) and (60.77,141.5) .. (79,141.5) .. controls (97.23,141.5) and (112,148.44) .. (112,157) .. controls (112,165.56) and (97.23,172.5) .. (79,172.5) .. controls (60.77,172.5) and (46,165.56) .. (46,157) -- cycle ;
%Curve Lines [id:da3822785661200183] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (79,121) .. controls (86,99) and (57,66) .. (138,70) ;
\draw [shift={(138,70)}, rotate = 2.83] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (0,7.27) -- (0,-7.27)(14.21,-6.37) .. controls (9.04,-2.99) and (4.3,-0.87) .. (0,0) .. controls (4.3,0.87) and (9.04,2.99) .. (14.21,6.37)   ;
%Curve Lines [id:da6469213883845986] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (79,193) .. controls (81,228) and (70,238) .. (136,238) ;
\draw [shift={(136,238)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (0,7.27) -- (0,-7.27)(14.21,-6.37) .. controls (9.04,-2.99) and (4.3,-0.87) .. (0,0) .. controls (4.3,0.87) and (9.04,2.99) .. (14.21,6.37)   ;
%Straight Lines [id:da801260302077782] 
\draw    (112,157) -- (262.15,207.05) ;
\draw [shift={(265,208)}, rotate = 198.43] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Flowchart: Decision [id:dp6183514662803711] 
\draw   (444.5,143) -- (482,167.75) -- (444.5,192.5) -- (407,167.75) -- cycle ;
%Shape: Rectangle [id:dp08599052194293733] 
\draw   (511,120.5) -- (655,120.5) -- (655,224.5) -- (511,224.5) -- cycle ;
%Shape: Ellipse [id:dp1625581422336697] 
\draw   (516,171.5) .. controls (516,152.72) and (546.22,137.5) .. (583.5,137.5) .. controls (620.78,137.5) and (651,152.72) .. (651,171.5) .. controls (651,190.28) and (620.78,205.5) .. (583.5,205.5) .. controls (546.22,205.5) and (516,190.28) .. (516,171.5) -- cycle ;
%Straight Lines [id:da20131284214872025] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (482,167.75) -- (510,167) ;
%Straight Lines [id:da9276346438749137] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (407,167.75) -- (391,168) ;
\draw [shift={(391,168)}, rotate = 179.1] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (0,7.27) -- (0,-7.27)(14.21,-6.37) .. controls (9.04,-2.99) and (4.3,-0.87) .. (0,0) .. controls (4.3,0.87) and (9.04,2.99) .. (14.21,6.37)   ;
%Straight Lines [id:da36922960746848754] 
\draw    (583.5,205.5) -- (354.98,234.13) ;
\draw [shift={(352,234.5)}, rotate = 352.86] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da11598580259192715] 
\draw    (341,77) -- (580.59,136.77) ;
\draw [shift={(583.5,137.5)}, rotate = 194.01] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;

% Text Node
\draw (230,68) node [anchor=north west][inner sep=0.75pt]   [align=left] {Disposition};
% Text Node
\draw (207,135) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{74.55pt}\setlength\topsep{0pt}
\begin{center}
Tobacco Vaping\\Stance
\end{center}

\end{minipage}};
% Text Node
\draw (207,219) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{79.66pt}\setlength\topsep{0pt}
\begin{center}
Cannabis Vaping\\Stance
\end{center}

\end{minipage}};
% Text Node
\draw (235,282) node [anchor=north west][inner sep=0.75pt]   [align=left] {USER};
% Text Node
\draw (62,149) node [anchor=north west][inner sep=0.75pt]   [align=center] {Ties};
% Text Node
\draw (8,196) node [anchor=north west][inner sep=0.75pt]   [align=left] {FRIENDS};
% Text Node
\draw (410,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {RESIDES};
% Text Node
\draw (544,231) node [anchor=north west][inner sep=0.75pt]   [align=left] {LOCATION};
% Text Node
\draw (544,142) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{57.16pt}\setlength\topsep{0pt}
\begin{center}
Cannabis \\Legalization\\ Policy
\end{center}

\end{minipage}};


\end{tikzpicture}
